How Smart Are `Water Smart Landscapes'?

Understanding the effectiveness of alternative approaches to water conservation is crucially important for ensuring the security and reliability of water services for urban residents. We analyze data from one of the longest-running "cash for grass" policies - the Southern Nevada Water Authority's Water Smart Landscapes program, where homeowners are paid to replace grass with xeric landscaping. We use a twelve year long panel dataset of monthly water consumption records for 300,000 households in Las Vegas, Nevada. Utilizing a panel difference-in-differences approach, we estimate the average water savings per square meter of turf removed. We find that participation in this program reduced the average treated household's consumption by 18 percent. We find no evidence that water savings degrade as the landscape ages, or that water savings per unit area are influenced by the value of the rebate. Depending on the assumed time horizon of benefits from turf removal, we find that the WSL program cost the water authority about $1.62 per thousand gallons of water saved, which compares favorably to alternative means of water conservation or supply augmentation.

==> bill_cohort.tex <==
&\multicolumn{1}{c}{Spring}&\multicolumn{1}{c}{Summer}&\multicolumn{1}{c}{Fall}&\multicolumn{1}{c}{Winter}\\
\hline
WSL Area            &       -5.08\sym{***}&       -13.1\sym{***}&       -7.84\sym{***}&       -1.89\sym{***}\\
                    &      (0.28)         &      (0.66)         &      (0.40)         &      (0.21)         \\
before 3/03 $\times$ WSL Area&        2.15\sym{**} &        2.73         &        3.59\sym{**} &        0.90         \\
                    &      (0.66)         &      (1.42)         &      (1.10)         &      (0.49)         \\
3/03 to 12/06 $\times$ WSL Area&        1.56\sym{***}&        2.98\sym{***}&        1.53\sym{**} &        0.72\sym{**} \\
                    &      (0.30)         &      (0.61)         &      (0.50)         &      (0.24)         \\
1/07 to 12/07 $\times$ WSL Area&        0.20         &       -0.50         &       -0.20         &        0.39         \\
                    &      (0.31)         &      (0.66)         &      (0.47)         &      (0.25)         \\
\hline
\(R^{2}\)           &       0.026         &       0.060         &       0.031         &       0.017         \\
Households          &      52,564         &      52,564         &      52,564         &      52,564         \\
Observations        &     657,413         &     650,719         &     660,259         &     662,265         \\


==> summary_all.tex <==
WSL Area& Spring&       -26.4\sym{***}&      (0.95)&       -26.9\sym{***}&      (0.95)&       -27.7\sym{***}&      (1.14)\\
 & Summer&       -63.9\sym{***}&      (1.95)&       -64.5\sym{***}&      (1.94)&       -64.8\sym{***}&      (2.37)\\
 & Fall&       -41.8\sym{***}&      (1.42)&       -41.4\sym{***}&      (1.37)&       -41.0\sym{***}&      (1.64)\\
 & Winter&       -11.6\sym{***}&      (0.61)&       -12.2\sym{***}&      (0.64)&       -12.2\sym{***}&      (0.90)\\
\rule{0pt}{3ex} 
WSL Area& Spring&                     &            &        0.21\sym{*}  &      (0.10)&        0.14         &      (0.10)\\
$\times$ Age& Summer&                     &            &        0.22         &      (0.20)&        0.17         &      (0.19)\\
 & Fall&                     &            &       -0.16         &      (0.16)&       -0.12         &      (0.16)\\
 & Winter&                     &            &        0.24\sym{**} &     (0.077)&        0.26\sym{**} &     (0.086)\\
\rule{0pt}{3ex} 
WSL Area& Spring&                     &            &                     &            &        0.34         &      (3.75)\\
$\times$ Cohort 1& Summer&                     &            &                     &            &       -12.4         &      (7.03)\\
 & Fall&                     &            &                     &            &       -0.47         &      (7.06)\\
 & Winter&                     &            &                     &            &       -2.09         &      (4.03)\\
\rule{0pt}{3ex} 
WSL Area& Spring&                     &            &                     &            &        1.61         &      (1.35)\\
$\times$ Cohort 2& Summer&                     &            &                     &            &        1.37         &      (2.26)\\
 & Fall&                     &            &                     &            &       -0.87         &      (2.11)\\
 & Winter&                     &            &                     &            &       -0.27         &      (1.12)\\
\rule{0pt}{3ex} 
WSL Area& Spring&                     &            &                     &            &        0.37         &      (1.44)\\
$\times$ Cohort 3& Summer&                     &            &                     &            &       -2.02         &      (2.87)\\
 & Fall&                     &            &                     &            &      -0.065         &      (2.23)\\
 & Winter&                     &            &                     &            &        1.40         &      (1.19)\\
\cmidrule{2-8}
& Spring &\multicolumn{2}{c}{       0.122         } &\multicolumn{2}{c}{       0.122         } &\multicolumn{2}{c}{       0.122         }\\
& Summer &\multicolumn{2}{c}{       0.246         } &\multicolumn{2}{c}{       0.246         } &\multicolumn{2}{c}{       0.246         }\\
& Fall &\multicolumn{2}{c}{       0.173         } &\multicolumn{2}{c}{       0.173         } &\multicolumn{2}{c}{       0.173         }\\
& Winter &\multicolumn{2}{c}{       0.071         } &\multicolumn{2}{c}{       0.071         } &\multicolumn{2}{c}{       0.071         }\\
\bottomrule

